Improved Galactic Foreground Removal for B-Modes Detection with Clustering Methods

Characterizing the sub-mm Galactic emission has become increasingly critical especially in identifying and removing its polarized contribution from the one emitted by the Cosmic Microwave Background (CMB). In this work, we present a parametric foreground removal performed onto sub-patches identified in the celestial sphere by means of spectral clustering. Our approach takes into account efficiently both the geometrical affinity and the similarity induced by the measurements and the accompanying errors. The optimal partition is then used to parametrically separate the Galactic emission encoding thermal dust and synchrotron from the CMB one applied on two nominal observations of forthcoming experiments from the ground and from the space. Performing the parametric fit singularly on each of the clustering derived regions results in an overall improvement: both controlling the bias and the uncertainties in the CMB $B-$mode recovered maps. We finally apply this technique using the map of the number of clouds along the line of sight, $\mathcal{N}_c$, as estimated from HI emission data and perform parametric fitting onto patches derived by clustering on this map. We show that adopting the $\mathcal{N}_c$ map as a tracer for the patches related to the thermal dust emission, results in reducing the $B-$mode residuals post-component separation. The code is made publicly available.

==> adjacency.tex <==
\section{Spectral Clustering on HEALPIX maps} \label{sec:spectral}
In this section, we present an implementation of spectral clustering applied on images defined on  the full celestial sphere. We adopt maps following the \textsc{HEALPix}  scheme \citep{2005ApJ...622..759G,Zonca2019}.




\subsection{Adjacency from the Heat Kernel} \label{subsec:heat_healpix}

Let us denote by $X=(\mathbf{x}_1,\dots, \mathbf{x}_{n_{\rm pix} } ) $, a set of  normed-1  vectors (with $\mathbf{x}_i \in \mathbb{R}^3$), encoding the coordinates of each \textsc{HEALPix} pixel.
Given $X$ we can construct a matrix,$\Theta$, from  the scalar product $  \Theta  = X^T  X $.  It is a $n_{\rm pix} \times n_{\rm pix} $ matrix, with diagonal equal to $1$, and off-diagonal elements  encoding the scalar product estimated on pairs of pixels. 


\subsection{Adjacency from the Heat Kernel} \label{subsec:heat_healpix}

Let us denote by $X=(\mathbf{x}_1,\dots, \mathbf{x}_{n_{\rm pix} } ) $, a set of  normed-1  vectors (with $\mathbf{x}_i \in \mathbb{R}^3$), encoding the coordinates of each \textsc{HEALPix} pixel.  The cosine matrix, defined in eq.~\eqref{eq:theta}, can be defined  from  the scalar product $  \Theta  = X^T  X $.  It is a $n_{\rm pix} \times n_{\rm pix} $ matrix, with diagonal equal to $1$, and off-diagonal elements  encoding the scalar product estimated on pairs of pixels. 

By means of eq.~\eqref{eq:heat_kernel}, the  adjacency matrix $A$ reads as: 
\begin{equation}
    A \equiv\sum_{\ell =0} ^{+\infty } \frac{2\ell +1}{4\pi}   e^{-t \ell(\ell+1)} \mathcal{P}_{\ell}( \Theta),
\label{eq:adj_heat}
\end{equation}
where the $t$ parameter can be  associated by analogy to the pixel resolution of the map, $\sigma_{\rm pix}^2$.  This scale  sets a threshold  $\ell_{\rm max} $  to which we can stop the sum in eq.~\eqref{eq:adj_heat}. We find that $\ell_{\rm max} $ can be   chosen to satisfy the following threshold-criterion\footnote{The value of $10^{-7}$ is estimated by the fact that  for a given angular scale  $\sigma_{\rm pix}$, it corresponds a multipole  scale, so that for $\ell> \ell_{\rm max}$ the terms in the sum can be further neglected.  }:  
\begin{equation}
 \frac{2\ell_{\rm max}  +1}{4\pi}   e^{-\ell_{\rm max} (\ell_{\rm max} +1) \sigma_{\rm pix}^2} \leq 10^{-7}.
\label{eq:lmax}
\end{equation}  
This choice can be intuitively motivated   by the following argument: as  the heat kernel   encodes the amount of heat emanating from a source located  in $x$  to a neighbor $x'= x +\delta x$, in a time $t'>0$, similarly, we can associate a measure of adjacency (or affinity)  between two pixels  $x$ and $x'$ by \emph{propagating} the affinity  parametrized by a characteristic scale as $ \sigma_{\rm pix}$. In fact, we find that the smaller $ \sigma_{pix}$, the higher will be $\ell_{\rm max}$.
This threshold is achieved at   $\ell_{\rm max} \gtrsim  35$ for HEALPix gridding  at \texttt{nside=32}, with size $\sigma_{\rm pix} \sim1.83$ deg.


\begin{figure} 
    \centering
    \includegraphics[scale=.4, trim=0 .0cm 0 0 ,clip=true ]{figures/affinity_row.pdf}
    \caption{Adjacency as estimated in eq.~\eqref{eq:heat_kernel} relative to the pixel centered at $(\ell, b)= (0,30)$ deg Galactic coordinates. We recall the reader that $A_{ij}$ is a $n_{\rm pix} \times n_{\rm pix} $, so its rows and/or columns can be visualized as \textsc{HEALPix} maps.}
    \label{fig:kernel}
\end{figure}


\begin{figure} 
    \centering
    \includegraphics[scale=.65, trim=.7cm .6cm 0 .6cm, clip=true ]{figures/evals_deform.pdf}
    \caption{Eigenvalues of Laplacian matrix estimated  as   in eq.~\eqref{eq:deform}, for several choices of the scaling factor $\alpha$.}
    \label{fig:evals_deform}
\end{figure}

 \begin{figure*} 
    
     \includegraphics[scale=.38, trim=0cm 1.cm 0 .7cm, clip=true ]{figures/spherical_harm_0.pdf}
      
    \includegraphics[scale=.47, trim=0 2cm 0 2.2cm, clip=true]{figures/spherical_harm_1.0.pdf}
    \includegraphics[scale=.47,trim=0 4cm 0 4cm, clip=true]{figures/spherical_harm_2.0.pdf}
    \includegraphics[scale=.47
    ,trim=0 4.7cm 0 4cm, clip=true]{figures/spherical_harm_3.0.pdf}
     \caption{The first eigenvectors of $L$  corresponding to $\ell=0,\dots,3$ and assuming no uncertainty deformation (i.e. $\alpha=0$). The colorbar ranges for all the maps between $\pm 0.07$. }
     \label{fig:evec_heat}
 \end{figure*}
 
 \begin{figure*} 
    
     \includegraphics[scale=.38, trim=0cm 1.cm 0 .7cm, clip=true ]{figures/def_spherical_harm_0.pdf}
      
    \includegraphics[scale=.47, trim=0 2cm 0 2.2cm, clip=true]{figures/def_spherical_harm_1.0.pdf}
    \includegraphics[scale=.47,trim=0 4cm 0 4cm, clip=true]{figures/def_spherical_harm_2.0.pdf}
    \includegraphics[scale=.47
    ,trim=0 4.7cm 0 4cm, clip=true]{figures/def_spherical_harm_3.0.pdf}
     \caption{The first eigenvectors of $L$  corresponding to $\ell=0,\dots,3$ and with  uncertainty deformation ($\alpha=0.25$). The colorbar ranges for all the maps between $\pm 0.02$. }
     \label{fig:evec_heat_def}
 \end{figure*}
 


We show in Fig.~\ref{fig:kernel} a row of the affinity matrix $ A$ as defined in eq.~\eqref{eq:heat_kernel}. Notice that as expected  the definition of nearest-neighbours corresponds to the \emph{hottest}  area surrounding a given pixel.  Given the definition of adjacency as in eq.~\eqref{eq:adj_heat}, we can therefore estimate the Laplacian matrix as in eq.~\eqref{eq:laplacian_sym}. 

Once the Laplacian matrix is built, we can estimate its      eigenvectors  related to the first $N_{eigen}$ smallest eigenvalues. 
We remark that we do not factorize the whole Laplacian matrix, since we are  interested in a subset of  eigenvectors.  We thus  approximate the  eigenpairs by means of the so called  \emph{ Ritz approximation}, a technique  which has already been shown in previous  literature  \citep{szydlarski_2014,puglisi_2018} to approximate very well  the exact eigenpairs of a matrix  when a small tolerance threshold  ($\leq 10^{-12}$) is adopted \citep{puglisi_2018}. 
 


\subsection{Adjacency weighted with uncertainties} \label{subsec:unc}

When clustering methodologies are employed, it is very common to   ask oneself how the  adjacency described in Section~\ref{subsec:heat_healpix}  is affected  in presence of  the uncertainties in the measurements at a given pixel location. 
 E.g. let us assume that we have measurements of the modified-black-body   spectral index of dust emission, $\beta_d$, and its uncertainties, $\sigma_d \equiv \sigma (\beta_d)$.
 We require that two pixels encoding statistically compatible values of $\beta_d$ would be more easily associated together into a single cluster  with respect to  pixels with incompatible values.  
 
 In this section, we therefore want to identify a way to include into the  heat-kernel adjacency (eq.~\eqref{eq:adj_heat})  given the measurements  of realistic maps of foreground spectral parameters. For the following application,  we will use the map of the dust spectral index $\beta_d$ and the uncertainty map $\sigma_d $  obtained  from the \planck data processed  with the COMMANDER separation algorithm \citet{pldiffuse2015}.

Intuitively, we can distort   $A$ defined in eq.~\eqref{eq:adj_heat} with  a certain  weight given  by  the measurements  and the uncertainty of the parameter  at a given pixel location.
 Given the state of art data on Galactic  foregrounds in the sub-mm regime,   we consider  the measurements in each pixel $i$ to be  normally distributed around $\beta_{d,i}$   with a width given by its uncertainties,  $\sigma_{d,i}$  \citep{pldiffuse2015}. We therefore  generate a mock sample of  100 Gaussian random  numbers given the features $(\beta_{d,p},\sigma_{d,p})$, and we estimate the two-sample Kolmogorov-Smirnov (KS) test onto  pairs of different pixels $i$ and $j$. This allows us  to test the null hypothesis that  the distribution of $\beta_d^i$ values is drawn from the same underlying distribution as those of $\beta_d^j$ within an assumed confidence level. We repeat the test $100$ times, evaluate the statistical quantile $Q_{ij}$ of each  KS test, and set the median value all the KS tests, $Q_{ij}^{med}$  as the adjacency weight evaluated for the $ij$ pixel pair. Thus, if $Q_{ij}^{med}$ is   small enough to  reject the null hypothesis at a $2\sigma$ confidence level, the connection is  weighted with a  very  low   weight and it is unlikely that  the two  pixels will be associated into the same cluster.  On the other hand, when   $Q_{ij}^{med}\sim 1  $ we cannot reject the null hypothesis and the two pixels can be associated, as they are \emph{ parallel} in this metric.
 
 In order to combine the adjacency from the KS test and the one defined in eq.~\eqref{eq:adj_heat}, we can  treat the KS quantiles as cosines of an angle, so that,  a straightforward deformation of  the angles  defined in eq.~\eqref{eq:theta} can be:  
 \begin{equation}
     \Theta'   = \cos \left( \arccos (\Theta   ) + \alpha \left(1 - Q^{med}\right)\frac{\pi}{2} \right), 
     \label{eq:deform}
 \end{equation}
 where $0<\alpha\leq 0.5$ is a \emph{scaling factor} parameter that  weighs the relative contribution of the KS quantile similarity  with respect to the geometrical one (the proximity of two pixels on the sky).{ Values of $\alpha>0.5$ results into too large distortions that   break  the metric properties of eq.~\eqref{eq:deform} and make   the Laplacian  a singular matrix (see  next Subsect.~\ref{sec:clustering}).} The   updated cosine matrix $\Theta'  $ is then finally inserted into eq.~\eqref{eq:adj_heat} to evaluate the adjacency weights obtained from this distortion. 
 

 In Fig.~\ref{fig:evals_deform} we show the first 100 Ritz eigenvalues $\lambda$ of $L$ for different choices of $\alpha $. We firstly  notice that for the $\alpha=0$ case (solid blue) line, the   algebraic multiplicity  grows proportionally  with   $2 \ell +1$. This is somewhat   expected since for a given integer  $\ell$, which is an eigenvalue of   $\hat{L}^2$, its multiplicity goes as $2\ell +1$, in correspondence with the  eigenvectors  related  to the $m$ azimuthal  multipole number.   Furthermore, the eigenvectors shown in Fig.~\ref{fig:evec_heat} perfectly resemble the  spherical harmonics. Both the eigenvalue degeneracy as well as the morphology of the Laplacian eigenvectors represent a remarkable  validation test for the overall implementation described above.   
Moreover,  the distortion introduced by $\alpha \neq 0$  results  in breaking  the Laplacian eigenfunction algebraic multiplicity, so that the eigenspectrum becomes strictly increasing for higher values of $\alpha$.  Consequently, the eigenvectors as well deviate from the spherical harmonics, being more and more weighted by the Galactic emission spectral parameter and the  uncertainties as shown  in Fig.~\ref{fig:evec_heat_def} for the  scaling factor $\alpha=0.25$. The Laplacian eigenvectors present  an increasing number of   asymmetric  features: e.g. cold or hot inhomogeneities areas  in proximity of  the Galactic mid-plane.


This  {geometric construction}, obtained by using the uncertainties in the measurements,   introduces a \emph{key difference} with respect to the standard image segmentation approach in which the affinity of the pixels in the image is evaluated \emph{orthogonally} to the adjacency of the pixels (a graph of a function is treated as a transverse deformation of a regular domain). In this case, the image affinity of the pixels introduces a geometric deformation of the mutual positions of the points on $S^2$.  

==> spectra_image_segmentation.tex <==
\iffalse \subsection{Choice of a discrete integral kernel}  


\iffalse The Laplace-Beltrami-based construction described in the previous sections can be replicated with a closely related operator $e^{-t\Delta_g}:L^2(M)\longrightarrow L^2(M)$ called (for $t>0$) the \emph{ heat propagator}. Fredholm theory in this case is applied through a Green's function called the \emph{heat kernel} $G(x,y,t)$. Similarly to what is done with the Schr\"odinger equation, the heat kernel is a special solution of 
\begin{displaymath}
\Delta_g G(\mathbf{x},\mathbf{y},t) =\partial_t G(\mathbf{x},\mathbf{y},t),
\end{displaymath}
such that
\begin{displaymath}
G(\mathbf{x},\mathbf{y},t)=e ^{t\Delta_g} \delta (\mathbf{x}-\mathbf{y} ) .
\end{displaymath}

The heat kernel is commonly used to solve    the diffusion equation with a source term $f(x)$ and with boundary conditions in integral form: 

\begin{equation}
u(x,t)= e^{-t\Delta_g} f(x)=\int_M G(x,y,t)f(y)d\omega_g
\label{eq:DiffusionSolution}
\end{equation}



\noindent The heat propagator  inherits from the Laplace-Beltrami operator the  properties of being  a self-adjoint,  positive-definite and compact operator. 
%For $t>0$, we can write $e^{-t\Delta_g}=(e^{-\Delta_g})^t$ where $e^{-\Delta_g}$ is a compact self-adjoint with real discrete spectrum $\beta_0 \geq \beta_1\geq...\geq \beta_i \longrightarrow 0$.
Its  corresponding eigenfunctions form a complete orthonormal basis of $L^2(M)$.


In these terms, the eigenvalue problem for the heat propagator  can be formulated as:
\begin{equation}
e^{-t\Delta_g}\varphi_i=\beta_i^t \varphi_i
\label{eigenexp}
\end{equation}

Let us set $\lambda_i:=-ln(\beta_i)$. By construction $e^{-t\Delta_g}\varphi_i$ satisfies the heat diffusion equation or all $i$, then substituting Equation~\ref{eigenexp} we get:

$$ 0=L[e^{-t\Delta_g}\varphi_i]= e^{-\lambda_i t}(\Delta_g \varphi_i-\lambda_i\varphi_i).$$ 

This means that $\varphi_i$ are precisely the eigenfunctions of the Laplace-Beltrami operator with eigenvalues $\lambda_i$. As a consequence, the relevant properties that enable efficient image segmentation through the Laplace-Beltrami operator (a low Dirichlet energy embedding of $M$ in $\mathbb{R}^n$ can be defined by eigenfunctions of the operator) can be directly extended to the heat propagator. In particular we see that \begin{equation}G(x,y,t)=\sum_i e^{-\lambda_i t} \varphi_i(x)\varphi_i(y).\label{eq:tensor_eigenf}\end{equation}

An argument provided in \cite{belkin} derives Equation~\eqref{graphL} by discretising the heat propagator. By substituting in \ref{eq:DiffusionSolution} in \ref{eq:heat_diff} we get:

\begin{align*}
\Delta_g f(x)=\Delta_g u(x,0)=&\frac{\partial }{\partial t} \left(\int_M G(x,y,t)f(y)d\omega_g\right)_{t=0} \nonumber \\
\approx& -\frac{1}{t}\left( f(x)-\int_M G(x,y,t)f(y)d\omega_g\right) \\
\approx&-\frac{1}{t}\left( f(x_i)-\sum_j G(x,y,t)f(x_j)\right). 
\end{align*}

The overall coefficient $1/t$ does not affect the spectral structure of the expression in the brackets. This argument is in line with the above discussion on the heat propagator and again justifies the diagonal term in the discrete definitions of the discrete Laplacian based on diffusion arguments. 

Point-wise and spectral convergent discretizations of the heat propagator have been developed in the manifold learning theory of diffusion maps ( see \cite{coifman,singer,berry}). 
\begin{comment} 
It is well known that in $\mathbb{R}^3$ the heat kernel is expressed as : 
$$
G(\mathbf{x},\mathbf{y},t) = \left(\frac{1}{4\pi t}\right)^{3/2} \exp\left(  - \frac{\parallel \mathbf{x}-\mathbf{y} \parallel ^2}{4t}\right)
$$

%$G(\mathbf{x},\mathbf{y},0) = \delta (\mathbf{x}-\mathbf{y})$ . 

For this reason discrete constructions of the Laplace-Beltrami operator exploit global and local Gaussian kernels.\medbreak   
\end{comment} 




In our case images are  obtained from the full celestial sphere. If we write the heat equation into spherical coordinates (for more details we refer the reader to the discussion Appendix A and Equation~\eqref{eq:heat_diff})  and we assume $r=1$ , the Laplacian $\Delta_g$ on $S^2$ becomes: 
\begin{equation}
 \Delta =\frac{1}{  \sin \theta }\frac{\partial}{\partial {\theta} }  \left(\sin \theta \frac{\partial}{\partial {\theta} } \right) + \frac{1}{ \sin^2 \theta }\frac{\partial^2}{\partial{\phi^2 } } \equiv 
  -\hat{L}^2.   
\end{equation}
This corresponds to the square \emph{orbital angular  momentum}  operator  in quantum mechanics, i.e. $- \hat{L}^2$, whose eigenfunctions are the \emph{Spherical Harmonics} , $Y_{\ell m}$ and eigenvalues $-\ell(\ell+1)$. Similarly to what presented above, the heat propagator operator, $\exp{- \hat{L}^2 t }$   shares the same eigenfunctions and eigenvalues as $- \hat{L}^2$.

In view of Equation~\ref{eq:tensor_eigenf}, we can thus derive the heat kernel given the initial delta distribution in  spherical coordinates\footnote{As a comparison, we report here the heat kernel in  $\mathbb{R}^3$: 
$$
G(\mathbf{x},\mathbf{y},t) = \left(\frac{1}{4\pi t}\right)^{3/2} \exp\left(  - \frac{\parallel \mathbf{x}-\mathbf{y} \parallel ^2}{4t}\right)
$$ 
with  $G(\mathbf{x},\mathbf{y},0) = \delta (\mathbf{x}-\mathbf{y})$ . 
}: 


\begin{align}
G(\mathbf{x},\mathbf{y},t)=& \sum_{\ell =0} ^{+\infty } e^{-t \ell(\ell+1)}  \sum _{m=-\ell} ^{+\ell} Y_{\ell m}(\mathbf{x}) Y_{\ell m}^* (\mathbf{y}) \nonumber  \\ 
=& \sum_{\ell =0} ^{+\infty } \frac{2\ell +1}{4\pi}   e^{-t \ell(\ell+1)} \mathcal{P}_{\ell}(\Theta_{\mathbf{xy}}), 
\label{eq:heat_kernel}
\end{align} 

where we exploit in the last equality  the properties of spherical harmonics expressed as function of  \emph{Legendre polynomials} evaluated across the \emph{cosine matrix}, i.e. 
\begin{equation}
    \Theta_{\mathbf{xy}} = \cos\theta_{\mathbf{xy}} = \frac{\mathbf{x} \cdot\mathbf{y}} {\parallel \mathbf{x}\parallel \parallel \mathbf{y}\parallel }.
    \label{eq:theta}
\end{equation}
 

 \fi
 
